On Robust Mean Estimation under Coordinate-level Corruption

We study the problem of robust mean estimation and introduce a novel Hamming distance-based measure of distribution shift for coordinate-level corruptions. We show that this measure yields adversary models that capture more realistic corruptions than those used in prior works, and present an information-theoretic analysis of robust mean estimation in these settings. We show that for structured distributions, methods that leverage the structure yield information theoretically more accurate mean estimation. We also focus on practical algorithms for robust mean estimation and study when data cleaning-inspired approaches that first fix corruptions in the input data and then perform robust mean estimation can match the information theoretic bounds of our analysis. We finally demonstrate experimentally that this two-step approach outperforms structure-agnostic robust estimation and provides accurate mean estimation even for high-magnitude corruption.

==> sections/discussion.tex <==
\section{Discussion and Extensions}\label{sec:discussion}
We have shown that utilizing redundancy in the observed samples to counteract corruption in both real-world and synthetic data sets can substantially improve estimates of the mean of a distribution; when the level of corruption is below a threshold, these techniques do not require knowing the structure beforehand.

Our results could be extended by considering other forms of structure; our results here have been exclusive to distributions with linear structure. 
Though approximate linear structure is present in many data sets, more complex forms of structure may result in more accurate recovery of missing entries in real-world data as they could more accurately approximate the true structure of the distribution.

Our model of adversarial corruption could also be extended to allow both hidden and otherwise modified entries as well as random errors in the data. 
Our experimental results show that leveraging redundancy is beneficial when the data is only approximately structured, making these promising avenues of future investigation. 
A complete model would also take the computational budget of the defender into account. 
Finally, our results could be extended to statistics other than the mean and to models of the effect of structure-based imputation as preprocessing for learning algorithms.

==> sections/entryLevel.tex <==
\section{Coordinate-level Corruption}\label{sec:dentry}
In this section, we define the coordinate-level measure of distribution shift $\dentry$ and the adversaries considered in this work. 
We also compare the proposed measure and adversaries with total variation distance $\dtv$ and the standard $\epsilon$-fraction sample-level adversary considered in the robustness literature.
All results presented in this section apply to corruption that corresponds to both missing values and value replacements.

\subsection{Preliminaries}
For any two distributions $P$ and $Q$ on $\R^n$, the total variation distance between the two is defined as $\dtv(P, Q) = \sup_{A \subseteq \R^n} |P(A) - Q(A)|$. The coupling $\gamma$ of two distributions $P,Q$ is a joint distribution of $P$ and $Q$ such that the marginal distributions are $P, Q$. Denote the set of all possible couplings of $P,Q$ to be $\Gamma(P, Q)$. We focus on estimators with small Mahalanobis distance, i.e., $||\hat{\mu} - \mu||_{\Sigma} = |(\hat{\mu}-\mu)^T\Sigma^{-1}(\hat{\mu}-\mu)|^{1/2}$, because bounds on $\dtv$ between Gaussians imply bounds on the Mahalanobis distance, in which one can find bounds on $\ell_2$ distance.


\subsection{Corruption Models}\label{sec:corruption_models}

We consider that the observed data follows an adversarially corrupted distribution that lies within some $\epsilon$-ball from the true distribution according to a discrepancy $d$.
We consider that corruption occurs to $N$ samples first drawn from the true distribution $D$ and then corrupted.
Given $N$ samples $x_1, \dots, x_N$ from distribution $D$ on $\R^n$, the adversary is allowed to inspect the samples and perform one of the following corruptions:
\begin{itemize}
    \item \textbf{Sample-level adversary ($\Aone$)}: The adversary is allowed to remove up to $\epsilon\cdot N$ samples and replace them with arbitrary vectors.
    \item \textbf{Value-fraction adversary ($\Atwo$)}: The adversary is allowed to remove up to $\rho\cdot N$ values in each coordinate and replace them with arbitrary values.
    \item \textbf{Coordinate-fraction adversary ($\Athree$)}: The adversary is allowed to remove $\alpha$-fraction of the coordinates on average over the samples (up to $\alpha\cdot n \cdot N$ values in the data set) and replace them with arbitrary values.
\end{itemize}

Adversary $\Aone$ corresponds to the standard adversary associated with Huber's contamination model, which either corrupts a sample completely or leaves it intact.
Adversaries $\Atwo$ and $\Athree$ are more fine-grained and can corrupt only part of the entries of a sample. 
The difference between $\Atwo$ and $\Athree$ is that the fraction being hidden per coordinate is restricted for $\Atwo$, while $\Athree$ is able to focus all corruption on a single coordinate. Figure~\ref{fig:AdvCompare} provides examples of corruption under $\Aone$, $\Atwo$ and $\Athree$ with the same budget, i.e., $\alpha=\rho=\epsilon$.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figures/adversaries.jpg}
\caption{Examples of corruption under $\Aone$, $\Atwo$ and $\Athree$ when $\alpha=\rho=\epsilon$. Not that the number of corrupted entries are the same, but $\Aone$ is restricted to place them in the same samples, and $\Atwo$ can only corrupt a limited fraction per coordinate, while $\Athree$ is able to place them arbitrarily.}
\label{fig:AdvCompare}
\end{figure}

For sufficiently large sample size, we can use the total variation distance $\dtv$ to quantify the shift of the distribution introduced by $\Aone$, which is $\dtv(D, D') \le \epsilon$, where $D'$ is the distribution after corruption.
However, for $\Atwo$ and $\Athree$, $\dtv$ would be misleading because a sample with one missing coordinate and a sample with many missing coordinates could be considered equally corrupted under it. 
It is more appropriate to differentiate between these cases and model corruption based on each coordinate than whole samples. 
Thus, we propose a new type of metric, referred to as $\dentry$, which can be used to measure coordinate-level corruption.

\begin{definition}[$\dentry$]\label{def:dentry}
For $x,y \in \R^n$, define $I(x,y) = [\mathbbm{1}_{x_1\neq y_1}, \dots, \mathbbm{1}_{x_n\neq y_n}]^\top$, an indicator for each coordinate. For distributions $D_1, D_2$ on $\R^n$,
\begin{align*}
\dentry^1(D_1, D_2) &= \inf_{\gamma \in \Gamma(D_1, D_2)} 
\frac{1}{n}\|\E_{(x,y)\sim \gamma}\left[I(x,y)\right]\|_1 \\
\dentry^\infty (D_1, D_2) &=  \inf_{\gamma \in \Gamma(D_1, D_2)} \|\E_{(x,y)\sim \gamma}\left[I(x,y)\right] \|_\infty
\end{align*}
\end{definition}

\begin{figure}[ht]
\centering
\includegraphics[width=0.8\textwidth]{figures/dtv_dentry.jpg}
\caption{A comparison of the distribution shift metrics under 2-dimensional uniform distribution. Note that the two shifts have the same $\dtv$ but different $\dentry$.}
\label{fig:disCompare}
\end{figure}

We illustrate a comparison of $\dentry$ and $\dtv$ in Figure~\ref{fig:disCompare}. $\dentry$ can describe the distribution shift due to corruptions introduced by adversaries $\Atwo$ and $\Athree$.
Specifically, the maximum distance that $\Atwo$ can shift $D$ by is $\dentry^\infty = \rho$. Similarly, the maximum distance that $\Athree$ can shift $D$ by is $\dentry^1 = \alpha$.
Next, we analyze the strength of adversaries $\Aone$, $\Atwo$, and $\Athree$ in more detail.

\subsection{Adversary Analysis and Comparison}\label{sec:advanalysis}

Adversaries $\Atwo$ and $\Athree$ are more fine-grained than the sample-level adversary $\Aone$ since they have the freedom to corrupt individual entries of the samples.
Similarly, $\Athree$ is more fine-grained than $\Atwo$.
As a result, the \emph{strength} of $\Atwo$ and $\Athree$, i.e., the magnitude of the distribution shift they can introduce, can vary in a wider range than that of $\Aone$.
We next provide a more detailed comparison of these three adversaries in terms of strength (1) for arbitrary distributions and (2) in the presence of highly structured data.

\newparagraph{Arbitrary distributions}
We first consider the case when the coordinate-level adversaries $\Atwo$ and $\Athree$ have limited budget and can corrupt a smaller number of samples than $\Aone$.
Formally, we have the next proposition.
\begin{proposition}
\label{lowerBoundAdversaryProposition}
If $\alpha,\, \rho \leq \epsilon / n$, then $\Aone$ can simulate $\Atwo$ and $\Athree$, and thus $\Aone$ is stronger.
\end{proposition}

% \begin{proof}
%     Suppose that $\Athree$ affects at least one entry in a subset $S$ of all samples. As at least one coordinate per sample is corrupted, $S$ must be at most an $\alpha$-fraction of all samples; since $\alpha \leq \epsilon / n$ the sample-level adversary can corrupt the entirety of every sample partially corrupted by the coordinate-level adversary, and thus, it is a stronger adversary given this condition. The proof for $\Atwo$ is similar.
% \end{proof}

In the same way, when $\alpha,\, \rho \ge \epsilon$, $\Atwo$ and $\Athree$ can simulate sample-level corruptions. Furthermore, we show how the strength of $\Atwo$ and $\Athree$ compare.

\begin{proposition}
\label{adversaryLemma}
If $\alpha,\, \rho \geq \epsilon$, then $\Atwo$ and $\Athree$ are stronger than $\Aone$. If $\alpha \ge \rho$, $\Athree$ is stronger than $\Atwo$. If $\alpha \le \rho / n$, $\Atwo$ is stronger than $\Athree$.
\end{proposition}
% \begin{proof}
%     If $\alpha,\, \rho \geq \epsilon$, similarly to the proof of Proposition \ref{lowerBoundAdversaryProposition}, $\Atwo$ and $\Athree$ can simulate $\Aone$ by placing all its corruptions on the $\epsilon N$ coordinates corrupted by $\Aone$. If $\alpha \ge \rho$, $\Athree$ can simulate $\Atwo$ by corrupting the coordinates corrupted by $\Atwo$ since $\Atwo$ can never corrupt more than $\rho$-fraction of coordinates in expectation. On the other hand, if $\alpha \le \rho / n$, $\Atwo$ can corrupt whatever coordinates $\Athree$ decides to corrupt since $\Athree$ cannot corrupt more than $\alpha n$-fraction of one coordinate. Thus, the three statements hold.
% \end{proof}

Hence when $\alpha=\rho=\epsilon$, i.e. when the total number of missing entries are the same, both $\Atwo$ and $\Athree$ are stronger $\Aone$.
Directly from the definitions of $\Aone$ and $\Athree$ and Proposition~\ref{adversaryLemma}, we have that when $\alpha \geq \epsilon$, there are distributions for which the coordinate-level adversary $\Athree$ can corrupt $O(n)$-times more samples than adversary $\Aone$.

\newparagraph{Structured data}
The previous analysis shows that $\Athree$ is significantly stronger for arbitrary distributions.
However, the characterization due to Propositions~\ref{lowerBoundAdversaryProposition} and \ref{adversaryLemma} is quite loose as the gap between $\epsilon/n$ and $\epsilon$ is large.
This gap raises the natural question: Are there distributions for which this gap is more tight, and hence, we can restrict the power of the coordinate-level adversary $\Athree$ to be comparable to that of the sample-level adversary $\Aone$?

We show that for distributions that exhibit structure, i.e., redundancy across the coordinates of the observed samples, we can reduce the strength of the coordinate-level adversary to roughly that of the sample-level adversary.
This means that although the coordinate-level corruption model is more fine-grained and stronger, by using structure to our advantage, we can robustly estimate the mean roughly as accurately as that for sample-level corruption. 
We formalize the notion of structure next.



Assume samples $x_i \in \R^n$ lie in a low-dimensional subspace such that $x_i = Az_i$, where $D_z$ generates samples $z_i \in \R^r$ and $A \in \R^{n\times r}$ represents the structure. We consider that the data sample before corruption corresponds to $x = Az$ and assume that corruption is introduced in $x$.
Matrix $A$ introduces redundancy in the corrupted, observed data samples. 
This allows us to detect corruption that may be introduced in the data and in many cases allows us to recover the true value of corrupted entries, e.g., by solving a system of linear equations (see Section~\ref{sec:known_struct}).
In fact, we measure the strength of the redundancy that $A$ introduces by considering its row space.
Note that the coordinates of $x = Az$, and hence, the corrupted data, will exhibit high redundancy when many rows of $A$ span a small subspace.
Following this intuition, we define the following quantity to describe how tolerant $A$ is to retaining its row space.

\begin{definition}[$m_A$]
\label{def:ma}
Given a sample $x = Az$ with $A \in \R^{n\times r}$, we define $m_A$ to be the minimum number of rows one needs to remove from $A$ to reduce the dimension of its row space by one.
\end{definition}

As we show below, $m_A$ is the key quantity that quantifies how robust estimation can be against coordinate-level corruptions. 
For example, when $A$ is the identity matrix $I$ we have that $m_I = 1$ and hence we can remove any row and reduce its row space, thus, we have low redundancy.
On the other hand, for the matrix $A = \left[e_1, \dots, e_1\right]^\top$, we have that $m_A = n$ because we have to remove all $e_1$'s in $A$ to reduce the dimension of its row space.
Overall, it is not hard to see that $1 \leq m_A \leq n$.

We next show that the higher the value that $m_A$ takes for a matrix $A$, the weaker a coordinate-level adversary becomes due to the increased redundancy. 
Intuitively, the coordinate-level adversary has to spend more budget per sample to introduce corruptions that will counteract the redundancy introduced by matrix $A$. 
As a consequence, the coordinate-level adversary cannot alter the original distribution too far in total variation distance, leading to more accurate robust estimation techniques.
We have the following theorem.

\begin{theorem}
\label{linear}
Given two probability distributions $D_1, D_2$ on $\R^n$ with support in the range of the linear transformation $A$,
$$\frac{m_A}{n}\cdot \dtv(D_1, D_2)  \le \dentry (D_1, D_2) \le \dtv(D_1, D_2)$$
\end{theorem}
% \begin{proof}
%     First, we will show the case for $\dentry^1$. 
%     \begin{align*}
%         \dentry^1(D_1, D_2) &= \inf_{\gamma \in \Gamma(D_1, D_2)} 
%         \frac{\|\E_{(x,y)\sim \gamma}\left[I(x,y)\right]\|_1}{n}\\
%         &= \inf_{\gamma \in \Gamma(D_1, D_2)} \E_{(x,y)\sim \gamma}\left[\frac{||x - y||_0}{n}\right]\\
%         &\leq \inf_{\gamma \in \Gamma(D_1, D_2)} \Pr_{(x,y)\sim\gamma}\left[x\neq y\right]\\
%         &=  \dtv(D_1,D_2)
%     \end{align*}
    
%     Now, we can write $D_1 = F(D_1')$ and $D_2 = F(D_2')$ for some distributions $D_1'$ and $D_2'$ on $\R^r$.
    
%     Suppose that $x \not\in \ker(A)$. Now, suppose by way of contradiction that $\Pi_i\, Ax$ is nonzero for fewer than $m_A$ values of $i$. Call the rows of $A$ $v_0^T,\dots,v_{n-1}^T$ and let $S$ be the subspace of $\R^r$ spanned by the $v_i$. As $x \not\in \ker(A)$, $Ax$ is nonzero. Hence, $\langle x,\,v_i\rangle$ is nonzero for some $i$ so $\Pi_S\,x$ is nonzero.

%     Now, let $\mathcal{B}$ be a basis for $S$ containing $\Pi_S\,x$. Consider the subspace $S'$ of $S$ spanned by $\{v_i\mid \langle x,\,v_i\rangle = 0\}$. As $\Pi_{S'}\, x = 0$, $\Pi_S\,x$ cannot be an element of $S'$ and so  $\mathcal{B}$ is not a basis for $S'$. Thus, the dimension of $S'$ is less than that of $S$; as $\abs{\{v_i\}}-\abs{\{v_i\mid \langle x,\,v_i\rangle = 0\}} < m_A$ we have a contradiction of the definition of $m_A$. Thus, if $x\neq 0 \in \R^r$, $\Pi_i\, Ax$ must be nonzero for at least $m_A$ values of $i$, and hence $||Ax||_0 \geq m_A$.
    
%     Now, suppose that $(x,y)\sim\gamma$ for some $\gamma \in \Gamma(D_1,D_2)$. Then, $x = Ax'$ and $y = Ay'$ for some $x', y' \in \R^r$. If $x\neq y$, then $Ax' \neq Ay'$ so $x'-y' \not\in \ker(A)$. Thus 
%     $$||A(x'-y')||_0 \geq m_A$$ 
%     by the above, and so 
%     $$\E_{(x,y)\sim \gamma}\left[||x - y||_0\right] \geq m_A\Pr_{(x,y)\sim\gamma}\left[x\neq y\right]$$
    
%     Therefore, we have that
%     \begin{align*}
%         \dentry^1(D_1, D_2) &= \inf_{\gamma \in \Gamma(D_1, D_2)} 
%         \frac{\|\E_{(x,y)\sim \gamma}\left[I(x,y)\right]\|_1}{n}\\
%         &= \inf_{\gamma \in \Gamma(D_1, D_2)} \E_{(x,y)\sim \gamma}\left[\frac{||x - y||_0}{n}\right]\\
%         &\geq \inf_{\gamma \in \Gamma(D_1, D_2)} \frac{m_A}{n} \Pr_{(x,y)\sim\gamma}\left[x\neq y\right]\\
%         &= \frac{m_A}{n}\, \dtv(D_1,D_2)
%     \end{align*}
    
%     In the case of $\dentry^\infty$, the left hand side follows from above by using the fact that $\|x\|_1 \le n \|x\|_\infty$ for $x \in \R^n$. Then,
%     \begin{align*}
%         \dentry^\infty (D_1, D_2) &=  \inf_{\gamma \in \Gamma(D_1, D_2)} \|\E_{(x,y)\sim \gamma}\left[I(x,y)\right] \|_\infty \\
%         &= \inf_{\gamma \in \Gamma(D_1, D_2)} \max_{i} \Pr_{(x,y)\sim \gamma}\left[x_i \neq y_i\right] \\
%         &\leq \inf_{\gamma \in \Gamma(D_1, D_2)} \Pr_{(x,y)\sim\gamma}\left[x\neq y\right]\\
%         &=  \dtv(D_1,D_2)
%     \end{align*}
    
%     Therefore, the theorem holds for the $\dentry$ metric.
% \end{proof}
This theorem states that as $m_A \rightarrow n$, metric $\dentry$, which bounds the power of the coordinate-level adversaries, is almost equal to $\dtv$, which bounds the sample-level adversary.
We derive the following corollary.

\begin{corollary}
\label{boundingCorollary}
Suppose that $D$ is the original distribution on $\R^n$ with structure determined by matrix $A$. Let $D'$ be the observed distribution in the range of A under $\Athree$ with budget $\alpha$ (or under $\Atwo$ with budget of $\rho$) and let $\epsilon=\dtv(D, D')$. We have that:
$$\frac{m_A\epsilon}{n}\ \leq \alpha, \, \rho \leq \epsilon$$
\end{corollary}
Therefore, when we have structure, we can extend our results in Proposition \ref{lowerBoundAdversaryProposition} to more accurately characterize the relative strength of the two adversaries. 
The next proposition follows directly from Corollary \ref{boundingCorollary} and shows when the coordinate-level adversary is unable to replicate the corruption caused by the sample-level adversary.

\begin{proposition}
\label{structureLowerBoundAdversaryProposition}
If $\alpha, \, \rho \leq m_A\epsilon/n$, then a sample-level adversary of budget $\epsilon$ can simulate a coordinate-level adversary of budget $\alpha$ or $\rho$.
\end{proposition}

In summary, we have shown that the presence of redundancy in the observed data samples can limit the power of the more flexible coordinate-level adversary.
In the next sections, we will show that this redundancy allows us to devise robust estimators that enjoy better estimation accuracy guarantees than the standard filtering-based robust estimation methods inspired by sample-level corruption schemes.

==> sections/knownStructure.tex <==
\section{Robust Mean Estimation and Structure}
We consider the problem of mean estimation for Gaussian distributions and cases where data corruption corresponds to deletion. 
We show that the redundancy (structure) in the observed data can reduce the power of a coordinate-level adversary to approximately that of a sample-level adversary via structure-aware robust estimation techniques.
In Sections~\ref{sec:no_structure} and \ref{sec:known_struct}, we provide tight bounds for mean estimation under sample-level and coordinate-level corruption given no structure and the exact structure of $A$. 
We highlight that $m_A$ is the key quantity that determines these information-theoretic limits. 
Then, we show how to leverage structure when $A$ is unknown in Section~\ref{sec:UnknownStruct}.
Table~\ref{tab:summary} summarizes all results presented in this section.
All results hold for adversary budgets bounded away from $0.5$ and for a sufficiently large sample size $N$.
All proofs are deferred to the supplementary material.

\begin{table}
\small\center
\caption{A summary of the estimation error results presented in Section~\ref{sec:mean_estimation}. The reported results characterize $||\hat{\mu} - \mu||_{\Sigma}$ for Gaussians when the entries are less than a constant.}
\label{tab:summary}
\vskip 0.15in
\begin{threeparttable}
\begin{tabular}{lccc}
\toprule
Structure & $\Aone$ & $\Atwo$ & $\Athree$ \\
\midrule
No Structure & $\Theta(\epsilon)$ & $\Omega(\rho \sqrt{n})$, $O(\rho n)$ & $\Theta(\alpha n)$ \\
Known $A$& $\Theta(\epsilon)$ & $O(\rho \frac{n}{m_A})$ & $\Theta(\alpha \frac{n}{m_A})$\\
Unknown $A$& $\Theta(\epsilon)$ & $\Theta(\rho \frac{n}{m_A})^{*}$ & $\Theta(\alpha \frac{n}{m_A})^\#$ \\
\bottomrule
\end{tabular}
\begin{tablenotes}
      \small
      \item $^*$ When $\rho < \frac{m_A-1}{n + (m_A - 1)(m_A-2)}$ \ $^\#$ $\alpha < \frac{1}{n}$
\end{tablenotes}
\end{threeparttable}
\vskip -0.1in
\end{table}

\subsection{Mean Estimation with No Structure}\label{sec:no_structure}
When there is no structure to the data, the samples do not lie in a lower-dimensional space, i.e., we have that $x \sim \mathcal{N}(\mu, \Sigma)$ where $\Sigma$ is full rank. 
This problem then reduces to mean estimation of a non-degenerate Gaussian, which has been studied extensively in variants of the $\Aone$-corruption models. 
Here, we prove new tight bounds for mean estimation under adversaries $\Atwo$ and $\Athree$.
Specifically, we show that robust mean estimation is much harder under coordinate-level corruption when we do not have structure.  

Under sample-level corruption ($\Aone$) where $\epsilon$-fraction of samples is corrupted, it is well-known that any mean estimator $\hat{\mu}$ has to information-theoretically be $\Omega(\epsilon)$-far from the true mean $\mu$ in Mahalanobis distance with $\Sigma$. 
On the other hand, the Tukey median \cite{tukey1975mathematics} is a mean estimator where $\|\hat{\mu} - \mu\|_\Sigma = O(\epsilon)$. 
Although finding the Tukey median is computationally intractable in high dimensions, we know that it is an optimal estimator of $\Theta(\epsilon)$.

Under $\Athree$, who can corrupt $\alpha$-fraction of the coordinates in expectation, hidden coordinates cannot be recovered exactly using other visible coordinates because each dimension is independent of each other. 
Then, if $\alpha \ge 1/n$, $\Athree$ can concentrate all corruption in the first coordinate of all samples and, without recovery, we cannot get any estimate of the mean for that coordinate. 
Thus, the following theorem suggests that coordinate-level corruption is more difficult to tolerate than sample-level corruption.

\begin{theorem}
\label{noStructureA}
Let $0<\alpha n<1/2$ and $\Sigma \in \R^{n\times n}$ be a full rank covariance matrix. 
Given a set of i.i.d. samples from $D = \mathcal{N}(\mu, \Sigma)$ where the set is corrupted by $\mathcal{A}_3$ of budget $\alpha$, an algorithm that outputs a mean estimator $\hat{\mu}$ must satisfy $\|\hat{\mu} - \mu\|_\Sigma = \Omega(\alpha n)$. 
In fact, the Tukey median obtains error $\|\hat{\mu} - \mu\|_\Sigma = \Theta(\alpha n)$.
\end{theorem}
% \begin{proof}
% With a budget of $\alpha$, $\Athree$ can concentrate its corruption on one particular coordinate, say the first coordinate. 
% If $\alpha n \ge 1$, we will lose all information for the first coordinate, making mean estimation impossible. 
% Since $\alpha < 1/n$, $\Athree$ can corrupt $\alpha n$-fraction of first coordinates of all samples. 
% Since the marginal distribution with respect to the first dimension is a univariate Gaussian, information-theoretically any mean estimator of the first coordinate must be $\Omega(\alpha n)$-far from the true mean of the first coordinate.

% Now with a corrupted set of samples, only at most $\alpha n$-fraction of the samples will be corrupted on one or more coordinates. 
% Then the corrupted distribution $D' = \mathcal{N}(\mu', \Sigma)$ will have $\dtv(D, D') \le \alpha n$. 
% Therefore, the Tukey median $\hat{\mu}$ for the corrupted set of samples achieves error $\|\hat{\mu} - \mu\|_\Sigma = O(\alpha n)$. 
% \end{proof}

Under corruption models $\Aone$ and $\Athree$, there are optimal algorithms that achieve error guarantees of $\Theta(\epsilon)$ and $\Theta(\alpha n)$, respectively. 
If $\alpha = \epsilon$, we know that $\Athree$ is a stronger adversary than $\Aone$, and in terms of error guarantee, $\Athree$ can corrupt the mean with a multiplicative factor of $n$ more than $\Aone$. 
Therefore, when no structure is present in the data, there is a significant estimation gap between sample-level and coordinate-level corruption.


\subsection{Mean Estimation with Known Structure}\label{sec:known_struct}
We consider the case when we have full information of matrix $A$. 
Under sample-level corruption, structure does not help recover missing samples so the previous result of $\Theta(\epsilon)$ holds for $\Aone$. 
We now study how much can structure help with mean estimation under $\Atwo$ and $\Athree$ corruption.

% Given $\epsilon$-sample-corrupted samples, we cannot recover any of the $\epsilon$-fraction missing samples, so we must estimate the mean with only the remaining samples. Then what is the worst a sample-level adversary can do the data? This depends on the structure $A$. Without loss of generality, we can assume each row of $A$ has $l_2$-norm 1 since we can preprocess the data to normalize the rows. 


% \begin{theorem}
% Given $A \in \R^{n\times r}$ of rank $r$, let $x_1, \dots, x_N$ be the original $N$ samples where $N$ is sufficiently large. For the set of samples where $\epsilon$-fraction of samples are hidden entirely, there is an algorithm that can estimate $\mu$ with error up to $O(\epsilon\sqrt{\frac{n}{r}})$ best case and up to $O(\epsilon\sqrt{n})$ worst case, depending on $A$. This is information-theoretically optimal.
% \end{theorem}

% \begin{proof}
% WLOG, $\mu = 0$. For the first case where the adversary can corrupt $\epsilon$-fraction of the samples, the worst case is when $A$ is a matrix where all rows are $e_1$. Then, removing $\epsilon$-fraction of the samples will affect every dimension by $O(\epsilon)$ so for all dimensions, so total $l_2$ error will be $O(\epsilon\sqrt{n})$. The best case is when $A$ is a vertical stack of $n/r$ $I_{r\times r}$ matrices (or similarly several orthonormal matrices). The adversary's strongest move is to concentrate the corruption on the samples that are farthest in the direction of the largest eigenvector of $A$. Whatever $A$ might look like, there exists a lower bound to the adversary.

% \[\max_{\|\mu'\| \le \epsilon} \sum_{i=1}^n (A_i^\top \mu' )^2 \ge \epsilon^2\cdot \E_{z \sim S^{n-1}} \left[\sum_{i=1}^n (A_i^\top z )^2 \right] = \epsilon^2 \frac{n}{r}\]

% \noindent
% Thus, best case $\|\mu'\|_2 = O(\epsilon \sqrt{\frac{n}{r}})$ and worst case $O(\epsilon \sqrt{n})$.
% \end{proof}

With known matrix $A$, we can recover missing coordinates by solving a linear system of equations using the remaining coordinates in the sample and $A$. 
This process is computationally efficient to recover missing coordinates. 
If we can recover missing coordinates using structure, the best strategy of $\Atwo$ or $\Athree$ is to corrupt coordinates so that recovery is computationally difficult or even impossible. 
To this end, the adversary must corrupt at least $m_A$ coordinates for that sample to make coordinate recovery impossible. 
In fact, the following theorem shows that $m_A$ is the key structural quantity that captures the information-theoretic lower bound in robust estimation.

\begin{theorem}
\label{reductionThm}
Assume samples $x_i = Az_i$ where $Z \sim \mathcal{N}(\mu, I)$ and let $\alpha$ be the budget for $\Athree$. 
Given a set of samples corrupted by $\Athree$, an algorithm that outputs a mean estimator $\hat{\mu}$ must satisfy $\|\hat{\mu} - A\mu\|_{AA^\top} = \Omega(\frac{\alpha n}{m_A})$. 
The Tukey median obtains error $\|\hat{\mu} - A\mu\|_{AA^\top} = \Theta(\frac{\alpha n}{m_A})$.
\end{theorem}
% \begin{proof}
% Define $\epsilon$ be the fraction of samples that has at least one corrupted coordinate. Note that $\Athree$ must corrupt at least $m_A$ coordinates of a sample to make his corruptions non-recoverable. 
% Given that we can recover any sample with less than $m_A$ corrupted coordinates, we have that $\epsilon \le \frac{\alpha n}{m_A}$. 
% If $D$ is the original distribution on $\R^n$ and $D'$ is the observed distribution, then $\dtv(D, D') \le \epsilon$. Since $\dtv$ between the two Gaussians is less than or equal to $\epsilon$, the Tukey median algorithm achieves $\|\hat{\mu} - A\mu\|_{AA^\top} = O(\frac{\alpha n}{m_A})$.

% For the lower bound, $\Athree$ can corrupt $\frac{\alpha n}{m_A}$-fraction of the samples so that the coordinates are non-recoverable and shift part of the original distribution $D$ to anywhere along the axes of missing coordinates. 
% Then, the proof follows the lower bound proof for estimating the mean of a Gaussian corrupted by $\Aone$. 
% Hence, since we cannot distinguish between two Gaussians that share $1-\frac{\alpha n}{m_A}$ of mass, $\|\hat{\mu} - A\mu\|_{AA^\top} = \Omega(\frac{\alpha n}{m_A})$
% \end{proof}

Theorem \ref{reductionThm} shows that for a matrix $A$ where $m_A \approx n$, the multiplicative gap between mean estimation under $\Aone$ and $\Athree$ becomes nearly $1$. 
This bridged gap implies that leveraging structure by imputation reduces the strength of $\Athree$ (and also $\Atwo$) to roughly that of a sample-level adversary.

Consider a linear structure $A$ such that each row is sampled uniformly from the unit sphere $\mathcal{S}^{r-1}$. 
Then $A$ has rank $r$ and $m_A = n-r+1$ with probability $1$. 
Similarly, for the matrices considered in \cite{matrixCompletion}, $m_A= n-r+1$ for almost every $A$ with respect to the Lebesgue measure on $\R^{n\times r}$. 
Naturally $n \gg r$, so the estimation error for $\hat{\mu}$ is approximately $\Theta(\alpha )$, which is the bound for $\Aone$ when $\epsilon = \alpha$. 
Our main result shows that we can restrict the strength of a coordinate-level adversary to that of a sample-level adversary and is information-theoretically optimal.

==> sections/matrixCompletion.tex <==
\subsection{Mean Estimation with Unknown Structure}
\label{sec:UnknownStruct}

In the real world, we may not know the structure beforehand. 
Hence, we need to first learn the dependencies that exist between coordinates from the visible entries before we use them to impute the missing ones. 
When the dependencies are linear, there is a natural connection between matrix completion and missing entry imputation. 
In this section, we show how matrix completion can help robust mean estimation in the setting of Definition~\ref{def:ma} when $A$ is unknown but has $m_A = n-r+1$. 
We make the assumption of infinite samples in this section.

We focus on unique recovery as it has the same effects as exact imputation. 
Corollary 1 in \cite{matrixCompletion} gives the conditions in which we can uniquely recover a low rank matrix with missing entries.
This result goes beyond random missing values and considers deterministic missing-value patterns.
We state it here as the following lemma, with small changes made to adapt to our context where each sample can be viewed as one column of a matrix.

\begin{lemma}
\label{lemmaNowak}
Assume samples $x_i = Az_i$ where $Z \sim \mathcal{N}(\mu, I)$, and $A$ is unknown but has $m_A = n-r+1$. 
If there exist $r+1$ disjoint groups of $n-r$ samples, and in each group, any $k$ samples have at least $r+k$ dimensions which are not completely hidden, all the samples with at least $r$ visible entries can be uniquely recovered.
\end{lemma}

The key to matrix completion is learning the $r$-dimensional subspace spanned by the samples. 
The samples with more than $r$ visible entries provide some information to identify the subspace. 
Once the subspace is known, any sample with at least $r$ visible entries can be uniquely recovered.

If we consider the case where the data is corrupted by $\Athree$, we have the following result.

\begin{theorem}
\label{thm:unknownA3}
Assume samples $x_i = Az_i$ where $Z \sim \mathcal{N}(\mu, I)$, and $A$ is unknown. 
Under corruption $\Athree$ with budget $\alpha < \frac{1}{n}$, there exists an algorithm that obtains error $\|\hat{\mu} - A\mu\|_{AA^\top} = \Theta(\frac{\alpha n}{m_A})$.
\end{theorem}

Theorem \ref{thm:unknownA3} is based on Theorem \ref{reductionThm} and the following lemma.

\begin{lemma}
\label{lemma:unknownA3}
Assume samples $x_i = Az_i$ where $Z \sim \mathcal{N}(\mu, I)$, and $A$ is unknown. 
When the data are corrupted by $\Athree$ with budget $\alpha$, if $\alpha \geq \frac{1}{n}$, we cannot recover any of the samples in the worst case, otherwise we can recover all the samples with less than $m_A$ missing entries.  
\end{lemma}

% \begin{proof}
% The adversary can simply hide one coordinate completely to prevent us from recovering that coordinate if at least one missing coordinate per sample in expectation is allowed. 
% If the expected number of missing coordinates per sample is less than one, there must then be some positive fraction of samples with no missing coordinates; as we have infinite samples, we can select any $r+1$ disjoint sets of $n-r$ such samples to satisfy the conditions in Lemma \ref{lemmaNowak}.
% \end{proof}

%This result for $\Athree$ appears trivial and uninteresting. Therefore, we pose additional restrictions on the adversary. We assume that the adversary can hide up to a fraction of $\rho$ of each coordinate, which is exactly the $\Atwo$ setting. We show that in the presence of $\Atwo$ corruption, we can achieve unique recovery as long as $\rho \leq \frac{1}{m_A-1}$ and each sample has at least $n-m_A+2$ visible entries.

If the data is corrupted by $\Atwo$, we have the following result.

\begin{theorem}
\label{thm:unknownA2}
Assume samples $x_i = Az_i$ where $Z \sim \mathcal{N}(\mu, I)$, and $A$ is unknown but has $m_A = n-r+1$. Under corruption $\Atwo$ with budget $\rho < \frac{m_A-1}{n+(m_A-1)(m_A-2)}$, there exists an algorithm that obtains error $\|\hat{\mu} - A\mu\|_{AA^\top} = \Theta(\frac{\rho n}{m_A})$.
\end{theorem}

Note that the threshold of the budget in Theorem \ref{thm:unknownA2} is greater than or equal to the threshold in Theorem \ref{thm:unknownA3}. 
Similar to Theorem \ref{thm:unknownA3}, Theorem \ref{thm:unknownA2} can be obtained from Theorem \ref{reductionThm} and the following lemma. Theorem \ref{reductionThm} can be applied here because $\Athree$ can simulate $\Atwo$.

\begin{lemma}\label{lm:recovery_rho}
When the data are corrupted by $\Atwo$ with budget $\rho$, if $\rho \geq \frac{m_A-1}{n}$, we cannot recover any of the samples in the worst case; if $\rho < \frac{m_A-1}{n+(m_A-1)(m_A-2)}$, we can recover all the samples with at least $r$ visible entries.  
\end{lemma}

% \begin{proof}
% First, We introduce the concept of hidden patterns. 
% The set of coordinates missing from a sample forms its hidden pattern. 
% We only consider the hidden patterns which have been applied to infinitely many samples as if only finitely many samples share a pattern, the adversary could hide those samples completely with $0$ budget. %We use $M$ to denote the number of distinct patterns which are shared by infinitely many samples, and $p_l$ to denote the probability of the $l^{th}$ pattern $P_l$, $l = 1,2,\dots, M$.

% When $\rho \geq \frac{m_A-1}{n}$, the adversary is able to hide $m_A-1$ entries for every sample, and we cannot learn the structure from samples with only $r$ visible entries.

% When $\rho < \frac{m_A-1}{n}$, the adversary does not have enough budget to hide $m_A-1$ entries of all the samples, so there exist some patterns with at least $r+1$ coordinates visible. 
% We use $M$ to denote the number of such patterns, and $p_l$ to denote the probability of the $l^{th}$ pattern $P_l$, $l = 1,2,\dots, M$.

% Next, we show a necessary condition for the adversary to prevent us from learning the structure. 
% Since we have infinitely many samples, one group of $n-r$ samples satisfying the conditions in Lemma \ref{lemmaNowak} is enough to learn the structure since we can find another $r$ groups by choosing samples with the same hidden patterns.

% It is obvious that the adversary has to hide at least one coordinate per pattern, otherwise we have infinitely many samples without corruption. 
% No matter what the patterns the adversary provides, we try to get the samples satisfies the conditions in Lemma \ref{lemmaNowak} by the following sampling procedure.

% \begin{enumerate}
% \item Start with one of the patterns, pick $r+1$ visible coordinates of it to form the initial visible set $V_1$. Take one sample from this pattern to form the initial sample group $G_0$. Mark this pattern as checked.
% \item For $K = 1,2,3,\dots, M-1$, take one of the unchecked patterns and check if it contains at least one visible coordinate not in $V_K$, the current visible set. If so, take one sample $x_K$ from it and pick any one of its visible coordinates $v_K \notin V_K$. Add $x_K$ to the sample group and $v_K$ to the visible set: $G_{K+1} = G_{K} \cup \{ x_K \}$, $V_{K+1} = V_{K} \cup \{ v_K \}$. If not, skip it. Mark the pattern as checked.
% \end{enumerate}

% We show by induction that any $k (k \leq K)$ different samples in $G_K$ have at least $r+k$ coordinates in $V_K$ not completely hidden. It is trivial that the property holds for $K = 1$. Assume that the property holds for $K$. According to the sampling procedure, when a new sample $x_K$ comes, it has at least one visible coordinate $v_K$ not in $V_K$. Consider any $k (k \leq K+1)$ different samples in $G_{K+1}$. If the $k$ samples don't include the new sample $x_K$, by the induction assumption they have at least $r+k$ coordinates in $V_K \subset V_{K+1}$ not completely hidden. If $x_K$ is one of the $k$ samples, again by the induction assumption the other $k-1$ samples have at least $r+k-1$ coordinates in $V_K$ not completely hidden, plus $v_K$ of $x_K$ is also not hidden, so there are at least $r+k$ coordinates in $V_{K+1}$ not completely hidden. Thus, the property also holds for $K+1$. By induction, any $k$ distinct samples from the group we get at the end of step 2 have at least $r+k$ coordinates not completely hidden, which means if the group has at least $n-r$ samples, the conditions in Lemma \ref{lemmaNowak} can be satisfied.

% Denote the set of the patterns being picked as $\mathcal{P}_P$ and the set of the patterns being skipped as $\mathcal{P}_S$. Based on the previous analysis, the adversary has to manipulate the patterns so that $|\mathcal{P}_P| \leq n-r-1$, in which case the visible set cannot cover all the coordinates, which means there exists at least one common hidden coordinate for the patterns in $\mathcal{P}_S$ (otherwise the pattern where that coordinate is visible should have been picked). Since the fraction of hidden entries in that common coordinate is less than or equal to $\rho$, the sum of the probabilities of the patterns in $\mathcal{P}_S$ satisfies $\sum_{l: P_l \in \mathcal{P}_S} p_l \leq \rho$. Since all the patterns have at least one missing coordinate, we also have $p_{l:P_l \in \mathcal{P}_P} \leq \rho$. Thus, we have $\sum_{l=1}^{M}p_l \leq (n-r) \rho$. In such a case, the overall fraction of missing entries $\eta$ satisfies
% \begin{align*}
% \eta &\geq \sum_{l=1}^{M}p_l \frac{1}{n} + (1-\sum_{l=1}^{M}p_l) \frac{n-r}{n} \\
%      &\geq (n-r) \rho \frac{1}{n} + (1-(n-r)\rho) \frac{n-r}{n}
% \end{align*}

% The first inequality holds because for the samples with at least $r+1$ visible entries, there are at least $1$ missing entries per sample, and for the samples with less than $r+1$ visible entries, there are at least $n-r$ missing entries per sample. In addition, $\eta$ also satisfies $\eta \leq \rho$, so we have $\rho \geq \frac{n-r}{n+(n-r-1)(n-r)} = \frac{m_A-1}{n+(m_A-1)(m_A-2)}$, which is a necessary condition for the adversary. Thus, if $\rho < \frac{m_A-1}{n+(m_A-1)(m_A-2)}$, we can learn the structure and impute all the samples with at least $r$ visible entries.
% \end{proof}

In summary, the above show that when the budget of the coordinate-level adversaries is bounded we can design structure-aware robust mean estimation methods even when the structure of $A$ is unknown.

%\begin{lemma}
%\label{patternNum}
%Assume each pattern hides at least one coordinate. With budget $\rho$, the adversary has to provide at least $\left\lceil \frac{1}{\rho} \right\rceil$ different patterns.
%\end{lemma}

%\begin{proof}
%We show that it is impossible to have fewer than $\left\lceil \frac{1}{\rho} \right\rceil$ different pattern with budget $\rho$. When the number of different patterns $M \leq \left\lceil \frac{1}{\rho} \right\rceil - 1$, the adversary would need budget $\rho' \geq \max \{ p_1, p_2, \dots, p_{M} \} \geq \frac{1}{M} \geq \frac{1}{\left\lceil \frac{1}{\rho} \right\rceil - 1} > {\rho}$.
%\end{proof}

%Based on Lemma \ref{lemmaNowak} and Lemma \ref{patternNum}, we have the following theorem.

%\begin{theorem}
%If $\rho \leq \frac{1}{m_A-1}$, and each sample has at least $n-m_A+2$ visible entries, almost all the samples can be uniquely recovered.
%\end{theorem} 

%\begin{proof}
%Since we have infinitely many samples, one group of $n-r$ samples satisfying the conditions in Lemma \ref{lemmaNowak} is enough since we can find another $r$ groups by choosing samples with the same hidden patterns. Next, we show that such a group of samples can always be found.

%If there exist a pattern with no coordinate being hidden, we can pick $n-r$ samples from that pattern to form such a group.

%If there is at least one coordinate being hidden per pattern, from Lemma \ref{patternNum} we know that there must be at least $n-r$ patterns because $\rho \leq \frac{1}{m_A-1} = \frac{1}{n-r}$. We also have $p_l \leq \frac{1}{n-r}$ for $l = 1,2,\dots, M$, because if the probability of any pattern is greater than $\frac{1}{n-r}$, the adversary doesn't have enough budget to hide any coordinate of that pattern. Since each sample has at least $n-m_A+2 = r+1$ visible entries, we can find one group of samples satisfying the conditions by the following sampling procedure.
%\begin{enumerate}
%\item Start with one of the patterns, pick $r+1$ visible coordinates of it to form the initial visible set $V_1$. Take one sample from this pattern to form the initial sample group $G_0$. Mark this pattern as checked.
%\item For $K = 1,2,3,\dots, M-1$, take one of the unchecked patterns and check if it contains at least one visible coordinate not in $V_K$, the current visible set. If so, take one sample $x_K$ from it and pick any one of its visible coordinates $v_K \notin V_K$. Add $x_K$ to the sample group and $v_K$ to the visible set: $G_{K+1} = G_{K} \cup \{ x_K \}$, $V_{K+1} = V_{K} \cup \{ v_K \}$. If not, skip it. 
%\item If the sample group contains $n-r$ samples, finish the procedure. If not, take one sample from any of the patterns being skipped, and add it to the sample group.
%\end{enumerate}

%Next we prove that the sample group constructed this way satisfies the unique recovery conditions in Lemma \ref{lemmaNowak}. 

%We show by induction that any $k (k \leq K)$ different samples in $G_K$ have at least $r+k$ coordinates in $V_K$ not completely hidden. It is trivial that the property holds for $K = 1$. Assume that the property holds for $K$. According to the sampling procedure, when a new sample $x_K$ comes, it has at least one visible coordinate $v_K$ not in $V_K$. Consider any $k (k \leq K+1)$ different samples in $G_{K+1}$. If the $k$ samples don't include the new sample $x_K$, by the induction assumption they have at least $r+k$ coordinates in $V_K \subset V_{K+1}$ not completely hidden. If $x_K$ is one of the $k$ samples, again by the induction assumption the other $k-1$ samples have at least $r+k-1$ coordinates in $V_K$ not completely hidden, plus $v_K$ of $x_K$ is also not hidden, so there are at least $r+k$ coordinates in $V_{K+1}$ not completely hidden. Thus, the property also holds for $K+1$. By induction, the sample group we get at the end of step 2 satisfies the unique recovery conditions.

%Finally we show that we can get $n-r$ samples at the end of step 2 in most cases, and in the only case when we cannot get that many samples, the sample group can still satisfies the unique recovery conditions after step 3. Denote the set of the patterns being picked as $\mathcal{P}_P$ and the set of the patterns being skipped as $\mathcal{P}_S$. If we don't get $n-r$ samples at the end of step 2, the visible set cannot cover all the coordinates, which means there exists at least one common hidden coordinate for the patterns in $\mathcal{P}_S$ (otherwise the pattern where that coordinate is visible should have been picked). Since the fraction of hidden entries in that common coordinate is less than or equal to $\frac{1}{n-r}$, the sum of the probabilities of the patterns in $\mathcal{P}_S$ satisfies $\sum_{l: P_l \in \mathcal{P}_S} p_l \leq \frac{1}{n-r}$, and then $\sum_{l : P_l \in \mathcal{P}_P} p_l \geq \frac{n-r-1}{n-r}$. Because $p_l \leq \frac{1}{n-r}$, we have $| \mathcal{P}_P | \geq n-r-1$, and the equality holds if and only if $p_l = \frac{1}{n-r}$ for all $l: P_l \in \mathcal{P}_P$. Thus, we cannot get $n-r$ samples only when all the probabilities of the patterns in $\mathcal{P}_P$ are $\frac{1}{n-r}$. However, in that case, all the hidden coordinates in any of the patterns in $\mathcal{P}_P$ should be visible in all the patterns in $\mathcal{P}_S$ because of the restriction on the hidden fraction. If we add one sample from any pattern in $\mathcal{P}_S$ to the sample group, any $k (k \leq n-r)$ samples in it including the last one we add will have no coordinate completely hidden, and thus the sample group satisfies the unique recovery conditions.

%\end{proof}

%In practice we can take the samples with less than $m_A$ missing entries and do matrix completion on them, since samples with less than $m_A-1$ missing entries provide information for learning the structure, and samples with exactly $m_A-1$ missing entries can be recovered if the structure is known. If those samples satisfy Lemma \ref{lemmaNowak}, they can be recovered exactly. The rest of the samples can be considered corrupted at sample level as they are not recoverable.  
